Enhanced Meta Label Correction for Coping with Label Corruption

Traditional methods for learning with the presence of noisy labels have successfully handled datasets with artificially injected noise but still fall short of adequately handling real-world noise. With the increasing use of meta-learning in the diverse fields of machine learning, researchers leveraged auxiliary small clean datasets to meta-correct the training labels. Nonetheless, existing meta-label correction approaches are not fully exploiting their potential. In this study, we propose an Enhanced Meta Label Correction approach abbreviated as EMLC for the learning with noisy labels (LNL) problem. We re-examine the meta-learning process and introduce faster and more accurate meta-gradient derivations. We propose a novel teacher architecture tailored explicitly to the LNL problem, equipped with novel training objectives. EMLC outperforms prior approaches and achieves state-of-the-art results in all standard benchmarks. Notably, EMLC enhances the previous art on the noisy real-world dataset Clothing1M by $1.52\%$ while requiring $\times 0.5$ the time per epoch and with much faster convergence of the meta-objective when compared to the baseline approach.

==> Extra/Tbl-training_times.tex <==
	\centering
	\begin{tabular}	{l | c | c }
        \toprule	 	
			\textbf{Method} & MLC & Ours \\
        \midrule
			\textbf{Epoch time} & 7.241h & 3.67h \\
		\bottomrule
	\end{tabular}

==> iccv2023AuthorKit/figures.tex <==



%%%%% MLC %%%%%%
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\label{fig:mlc}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,301); %set diagram left start at 0, and has height of 301

%Rounded Rect [id:dp1354708855331157] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.12 ] (125.56,60.9) .. controls (141.25,60.9) and (153.97,73.63) .. (153.97,89.32) -- (153.97,206.37) .. controls (153.97,222.07) and (141.25,234.79) .. (125.56,234.79) -- (40.3,234.79) .. controls (24.61,234.79) and (11.89,222.07) .. (11.89,206.37) -- (11.89,89.32) .. controls (11.89,73.63) and (24.61,60.9) .. (40.3,60.9) -- cycle ;
%Straight Lines [id:da5284623534004369] 
\draw    (103,262) -- (103.95,223) ;
\draw [shift={(104,221)}, rotate = 91.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6369761712918443] 
\draw    (54,264) -- (54,153) ;
\draw [shift={(54,151)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp8357955015596454] 
\draw  [draw opacity=0][fill={rgb, 255:red, 213; green, 151; blue, 225 }  ,fill opacity=1 ] (67,197) .. controls (67,193.69) and (69.69,191) .. (73,191) -- (136,191) .. controls (139.31,191) and (142,193.69) .. (142,197) -- (142,215) .. controls (142,218.31) and (139.31,221) .. (136,221) -- (73,221) .. controls (69.69,221) and (67,218.31) .. (67,215) -- cycle ;
%Rounded Rect [id:dp6423418088327659] 
\draw  [draw opacity=0][fill={rgb, 255:red, 255; green, 217; blue, 102 }  ,fill opacity=1 ] (36,119) .. controls (36,114.58) and (39.58,111) .. (44,111) -- (110,111) .. controls (114.42,111) and (118,114.58) .. (118,119) -- (118,143) .. controls (118,147.42) and (114.42,151) .. (110,151) -- (44,151) .. controls (39.58,151) and (36,147.42) .. (36,143) -- cycle ;
%Straight Lines [id:da9167594266290644] 
\draw    (104,191) -- (104,154) ;
\draw [shift={(104,152)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7491952501679651] 
\draw    (79,111.5) -- (79,38.5) ;
\draw [shift={(79,36.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (38,268) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle h( x_{i})$};
% Text Node
\draw (97,263) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \tilde{y}_{i}$};
% Text Node
\draw (71,197) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textbf{Embedding}}};
% Text Node
\draw (63,123) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small \textbf{MLP}}};
% Text Node
\draw (75,12) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle y$};

\end{tikzpicture}


%%% MPL %%%



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,301); %set diagram left start at 0, and has height of 301

%Rounded Rect [id:dp1354708855331157] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.12 ] (125.56,60.9) .. controls (141.25,60.9) and (153.97,73.63) .. (153.97,89.32) -- (153.97,206.37) .. controls (153.97,222.07) and (141.25,234.79) .. (125.56,234.79) -- (40.3,234.79) .. controls (24.61,234.79) and (11.89,222.07) .. (11.89,206.37) -- (11.89,89.32) .. controls (11.89,73.63) and (24.61,60.9) .. (40.3,60.9) -- cycle ;
%Straight Lines [id:da5284623534004369] 
\draw    (81,262) -- (80.52,204) ;
\draw [shift={(80.5,202)}, rotate = 89.52] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp6423418088327659] 
\draw  [draw opacity=0][fill={rgb, 255:red, 169; green, 209; blue, 142 }  ,fill opacity=1 ] (41.5,90) .. controls (41.5,87.24) and (43.74,85) .. (46.5,85) -- (113,85) .. controls (115.76,85) and (118,87.24) .. (118,90) -- (118,105) .. controls (118,107.76) and (115.76,110) .. (113,110) -- (46.5,110) .. controls (43.74,110) and (41.5,107.76) .. (41.5,105) -- cycle ;
%Straight Lines [id:da7491952501679651] 
\draw    (79.5,86) -- (79.02,38.5) ;
\draw [shift={(79,36.5)}, rotate = 89.42] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Manual Operation [id:dp49266236513669925] 
\draw  [draw opacity=0][fill={rgb, 255:red, 118; green, 214; blue, 255 }  ,fill opacity=1 ] (117,135) -- (136.5,200) -- (32.5,200) -- (52,135) -- cycle ;
%Straight Lines [id:da5242245574967093] 
\draw    (81.5,136) -- (81.5,112) ;
\draw [shift={(81.5,110)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (75,263) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle x_{i}$};
% Text Node
\draw (52,91) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\textbf{Classifier}};
% Text Node
\draw (75,12) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle y$};
% Text Node
\draw (51,152) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{46.6pt}\setlength\topsep{0pt}
\begin{center}
\textbf{ResNet}\\\textbf{Backbone}
\end{center}

\end{minipage}};


\end{tikzpicture}


%%%%%% Strong Teacher %%%%%


\begin{figure}
\centering

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,479); %set diagram left start at 0, and has height of 479

%Rounded Rect [id:dp9500709104974059] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.12 ] (322.57,57.09) .. controls (362.11,57.13) and (394.14,89.21) .. (394.1,128.76) -- (393.9,358.4) .. controls (393.87,397.94) and (361.79,429.97) .. (322.24,429.93) -- (107.44,429.75) .. controls (67.9,429.71) and (35.87,397.63) .. (35.9,358.08) -- (36.1,128.44) .. controls (36.14,88.9) and (68.22,56.87) .. (107.76,56.91) -- cycle ;
%Straight Lines [id:da3273977273856765] 
\draw    (291,439) -- (291,382) ;
\draw [shift={(291,380)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da005016521403587326] 
\draw    (97,449) -- (97,381) ;
\draw [shift={(97,379)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp33547377934360423] 
\draw  [draw opacity=0][fill={rgb, 255:red, 213; green, 151; blue, 225 }  ,fill opacity=1 ] (246,349.6) .. controls (246,345.4) and (249.4,342) .. (253.6,342) -- (329.4,342) .. controls (333.6,342) and (337,345.4) .. (337,349.6) -- (337,372.4) .. controls (337,376.6) and (333.6,380) .. (329.4,380) -- (253.6,380) .. controls (249.4,380) and (246,376.6) .. (246,372.4) -- cycle ;
%Rounded Rect [id:dp49187042250251056] 
\draw  [draw opacity=0][fill={rgb, 255:red, 255; green, 217; blue, 102 }  ,fill opacity=1 ] (161,191.4) .. controls (161,186.76) and (164.76,183) .. (169.4,183) -- (267.6,183) .. controls (272.24,183) and (276,186.76) .. (276,191.4) -- (276,216.6) .. controls (276,221.24) and (272.24,225) .. (267.6,225) -- (169.4,225) .. controls (164.76,225) and (161,221.24) .. (161,216.6) -- cycle ;
%Straight Lines [id:da8548724589970478] 
\draw    (291,340) -- (291,333) -- (291,316) ;
\draw [shift={(291,314)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3791016071323665] 
\draw    (216,69) -- (216,33.5) ;
\draw [shift={(216,31.5)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Manual Operation [id:dp8787670027481016] 
\draw  [draw opacity=0][fill={rgb, 255:red, 118; green, 214; blue, 255 }  ,fill opacity=1 ] (123.84,314) -- (139.5,379) -- (56,379) -- (71.66,314) -- cycle ;
%Straight Lines [id:da06847077048393468] 
\draw    (97,315) -- (97,288) ;
\draw [shift={(97,286)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1794586847021986] 
\draw    (100,265) -- (100,227) ;
\draw [shift={(100,225)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp6837049511244295] 
\draw  [draw opacity=0][fill={rgb, 255:red, 169; green, 209; blue, 142 }  ,fill opacity=1 ] (59,191.4) .. controls (59,186.76) and (62.76,183) .. (67.4,183) -- (132.6,183) .. controls (137.24,183) and (141,186.76) .. (141,191.4) -- (141,216.6) .. controls (141,221.24) and (137.24,225) .. (132.6,225) -- (67.4,225) .. controls (62.76,225) and (59,221.24) .. (59,216.6) -- cycle ;
%Straight Lines [id:da6021189831403622] 
\draw    (100,257) -- (197,257) ;
%Straight Lines [id:da5820052203252057] 
\draw    (198,258) -- (198,226) ;
\draw [shift={(198,224)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2929752990627883] 
\draw    (100,183) -- (100,156) ;
\draw [shift={(100,154)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Or [id:dp7860540356312491] 
\draw   (198,87.5) .. controls (198,77.84) and (206.28,70) .. (216.5,70) .. controls (226.72,70) and (235,77.84) .. (235,87.5) .. controls (235,97.16) and (226.72,105) .. (216.5,105) .. controls (206.28,105) and (198,97.16) .. (198,87.5) -- cycle ; \draw   (198,87.5) -- (235,87.5) ; \draw   (216.5,70) -- (216.5,105) ;
%Straight Lines [id:da8075862522917974] 
\draw    (99,121) -- (99,87) ;
%Straight Lines [id:da4100836357198332] 
\draw    (99,87) -- (196,87.49) ;
\draw [shift={(198,87.5)}, rotate = 180.29] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da608629944453154] 
\draw    (351,88) -- (352,404) ;
%Straight Lines [id:da01558998681283108] 
\draw    (351,88) -- (286,88) -- (237,87.52) ;
\draw [shift={(235,87.5)}, rotate = 0.56] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da0676215373647786] 
\draw    (218,184) -- (218,156) ;
\draw [shift={(218,154)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da02341785016762188] 
\draw    (217,137) -- (216.53,107) ;
\draw [shift={(216.5,105)}, rotate = 89.1] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9848674243690032] 
\draw    (290,257) -- (290,295) ;
%Straight Lines [id:da5304209094572563] 
\draw    (236,257) -- (290,257) ;
%Straight Lines [id:da07375594956777531] 
\draw    (236,257) -- (236,227) ;
\draw [shift={(236,225)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8007546025351595] 
\draw    (290.5,405) -- (352,404) ;

% Text Node
\draw (90,450) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle x_{i}$};
% Text Node
\draw (284,443) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \tilde{y}_{i}$};
% Text Node
\draw (256,353) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textbf{Embedding}}};
% Text Node
\draw (204,195) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textbf{MLP}}};
% Text Node
\draw (132,2) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle y=w_{i} \cdot \tilde{y}_{i} +( 1-w_{i}) \cdot \hat{y}_{i}$};
% Text Node
\draw (70,333) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{37.83pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\footnotesize ResNet}}\\\textbf{{\footnotesize Backbone}}
\end{center}

\end{minipage}};
% Text Node
\draw (91,264) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle h_{i}$};
% Text Node
\draw (284,293) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle z_{i}$};
% Text Node
\draw (77,199) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\textbf{{\footnotesize Classifier}}};
% Text Node
\draw (94,129) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \hat{y}_{i}$};
% Text Node
\draw (208,135) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle w_{i}$};


\end{tikzpicture}

\end{figure}



